AGRAMPLIFIER: Defending Federated Learning Against Poisoning Attacks Through Local Update Amplification

The collaborative nature of federated learning (FL) poses a major threat in the form of manipulation of local training data and local updates, known as the Byzantine poisoning attack. To address this issue, many Byzantine-robust aggregation rules (AGRs) have been proposed to filter out or moderate suspicious local updates uploaded by Byzantine participants. This paper introduces a novel approach called AGRAMPLIFIER, aiming to simultaneously improve the robustness, fidelity, and efficiency of the existing AGRs. The core idea of AGRAMPLIFIER is to amplify the "morality" of local updates by identifying the most repressive features of each gradient update, which provides a clearer distinction between malicious and benign updates, consequently improving the detection effect. To achieve this objective, two approaches, namely AGRMP and AGRXAI, are proposed. AGRMP organizes local updates into patches and extracts the largest value from each patch, while AGRXAI leverages explainable AI methods to extract the gradient of the most activated features. By equipping AGRAMPLIFIER with the existing Byzantine-robust mechanisms, we successfully enhance the model's robustness, maintaining its fidelity and improving overall efficiency. AGRAMPLIFIER is universally compatible with the existing Byzantine-robust mechanisms. The paper demonstrates its effectiveness by integrating it with all mainstream AGR mechanisms. Extensive evaluations conducted on seven datasets from diverse domains against seven representative poisoning attacks consistently show enhancements in robustness, fidelity, and efficiency, with average gains of 40.08%, 39.18%, and 10.68%, respectively.

==> chapters/Bio.tex <==
% \section{Biography Section}
% If you have an EPS/PDF photo (graphicx package needed), extra braces are
%  needed around the contents of the optional argument to biography to prevent
%  the LaTeX parser from getting confused when it sees the complicated
 % $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
 % your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
 % simpler here.)
 
\vspace{11pt}

% \bf{If you include a photo:}
\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio-pics/Zirui_Gong.jpeg}}]{Zirui Gong} received the B.E degree (Honors) in information technology from Deakin University, VIC, Australia in 2023. She is currently working as a research assistant with the School of Information and Communication Technology, Griffith University, QLD, Australia, while also pursuing a Ph.D. opportunity. Her research interests include trustworthy AI and privacy-preserving in federated learning.

\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio-pics/Liyue_Shen.jpg}}]{Liyue Shen} received the bachelor's degree in Communication Science and Engineering from Fudan University, China, in 2014 and Master's degree in information technology from the University of Queensland in 2022. His research interest includes privacy preserving in federated learning.

\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio-pics/yanjun.jpg}}]{Yanjun Zhang} is currently a Lecturer with the School of Computer Science, University of Technology Sydney, NSW, Australia. She used to be a faculty member at the School of Information Technology, Deakin University, from 2022 to 2023. She received her Ph.D. degree from the University of Queensland in 2021. She also holds a research position with CSIRO’s Data61. Her current research focuses on trustworthy AI, security and privacy, and machine learning.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio-pics/Leo_Zhang.jpg}}]{Leo Yu Zhang} (M’17) is currently a Senior Lecturer with the School of Information and Communication Technology, Griffith University, QLD, Australia. He used to be a faculty member at the School of Information Technology, Deakin University, from 2018 to 2023. He received his Ph.D. degree from the City University of Hong Kong in 2016. He held various research positions with the City University of Hong Kong, the University of Macau, the University of Ferrara, and the University of Bologna. His current research focuses on trustworthy AI and applied cryptography, and he has published over 100 articles in refereed journals and conferences, such as TIFS, TDSC, Oakland, AsiaCCS, NeurIPS, CVPR, IJCAI, AAAI, etc.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio-pics/}}]{Jingwei Wang} is a postgraduate student at the School of Electrical Engineering and Computer Science, The University of Queensland, Australia. Contact him at jingwei.wang@uq.net.au.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio-pics/}}]{Guangdong Bai} is an Associate Professor at the School of Electrical Engineering and Computer Science, The University of Queensland, Australia. His research interests include cybersecurity, software engineering, and formal methods. Contact him at g.bai@uq.edu.au.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio-pics/}}]{Yong Xiang} 
\end{IEEEbiography}







\vspace{11pt}

% \bf{If you will not include a photo:}\vspace{-33pt}
% \begin{IEEEbiographynophoto}{John Doe}
% Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
% \end{IEEEbiographynophoto}




\vfill


==> chapters/problem.tex <==
\section{Problem formulation}

\subsection{Attack Model}
We evaluate the proposed \codename method against both untargeted attacks and targeted attacks. 
We consider an attack model which is in favor of the  poisoning adversary among prior research~\cite{bagdasaryan_how_2019,bhagoji_analyzing_2019,cao_fltrust_2022,jagielski_manipulating_2018}. 
% \yanjun{please help me to fill in the bibtex}. 
We allow the adversary to have the full knowledge of gradients generated by all participants, including those from benign ones. 
This enables the optimized and adaptive poisoning attacks and demonstrates compelling attack performance in recent studies~\cite{cao_fltrust_2022,jagielski_manipulating_2018}.
The attacker can take full control of a proportion of  clients, including their local updates, local training data %~\highlight{hyper parameters, local updates,}~\yanjun{I was wondering if you mean ``hyper parameters" or ``local parameters", or local updates (e.g., local gradients)?} \liyue{I'm thinking of all of them - attacker can full control, update to `` hyper parameters, local updates," } 
and hyperparameters.  
The attacker can also decide whether to inject malicious updates for the current round or not.
We assume the attacker does not compromise the central aggregator, following the literature of \agrs. 

%We follow the previous attack models: \emph{grad-ascent attack} \cite{kurakin_adversarial_2017,munoz-gonzalez_towards_2017}, \emph{label-flip attack} \cite{cao_fltrust_2022,fang_local_2021,li_lomar_2022}, \emph{min-max attack} \cite{noauthor_manipulating_nodate}, \emph{mislead attack} \cite{kurakin_adversarial_2017,li_lomar_2022}, \emph{scale attack} \cite{cao_fltrust_2022}, in which the malicious clients can send arbitrary local model updates to the server in each iteration of the FL training process. 
\subsection{Defense Model}
%We aim to design an FL aggregation algorithm that can 
The defense goal is to achieve Byzantine robustness against malicious clients as well as maintain its fidelity and efficiency. Specifically, the strategy should not compromise the global model's classification accuracy, and it should be able to learn a global model that is as accurate in non-adversarial conditions as the global model learned by FedAvg. Also, the method should retain computation efficiency and good scalability in large-scale FL training.  %shouldn't involve additional processing or communications costs for each client. Specifically, we record the attack success rate and test accuracy as indicators of robustness. We also examine the test accuracy under no attack scenario to examine the fidelity of the strategy. 

We consider the defense strategy to be implemented on the server side. The server can gather a clean small training dataset for FL training which is free of contamination. Since we only need a small clean dataset, e.g., 100 training examples, manual gathering and labeling on the server side is feasible. 
